Towards Scalable Quantum Networks

This paper presents a comprehensive study on the scalability challenges and opportunities in quantum communication networks, with the goal of determining parameters that impact networks most as well as the trends that appear when scaling networks. We design simulations of quantum networks comprised of router nodes made up of trapped-ion qubits, separated by quantum repeaters in the form of Bell State Measurement (BSM) nodes. Such networks hold the promise of securely sharing quantum information and enabling high-power distributed quantum computing. Despite the promises, quantum networks encounter scalability issues due to noise and operational errors. Through a modular approach, our research aims to surmount these challenges, focusing on effects from scaling node counts and separation distances while monitoring low-quality communication arising from decoherence effects. We aim to pinpoint the critical features within networks essential for advancing scalable, large-scale quantum computing systems. Our findings underscore the impact of several network parameters on scalability, highlighting a critical insight into the trade-offs between the number of repeaters and the quality of entanglement generated. This paper lays the groundwork for future explorations into optimized quantum network designs and protocols.

==> references.tex <==
@article{chehimi2023matching,
    title={Matching Game for Optimized Association in Quantum Communication Networks},
    author={Chehimi, Mahdi and Simon, Bernd and Saad, Walid and Klein, Anja and Towsley, Don and Debbah, Mérouane},
    year={2023}
}

@article{chehimi2023scaling,
    title={Scaling Limits of Quantum Repeater Networks},
    author={Chehimi, Mahdi and Pouryousef, Shahrooz and Panigrahy, Nitish K. and Towsley, Don and Saad, Walid},
    year={2023}
}

@article{farahbakhsh2023opportunistic,
    title={Opportunistic Routing in Quantum Networks},
    author={Farahbakhsh, Ali and Feng, Chen},
    year={2023}
}
https://www.overleaf.com/project/6532a2b0c3b75be2b8e6d5af

@article{shi2023quantumrouting,
    title={Quantum Routing for Emerging Quantum Networks},
    author={Shi, Wenbo and Malaney, Robert},
    year={2023}
}

@article{wu2021sequence,
  title={SeQUeNCe: a customizable discrete-event simulator of quantum networks},
  author={Wu, Xiaoliang and Kolar, Alexander and Chung, Joaquin and Jin, Dong and Zhong, Tian and Kettimuthu, Rajkumar and Suchara, Martin},
  journal={Quantum Science and Technology},
  volume={6},
  number={4},
  pages={045027},
  year={2021},
  publisher={IOP Publishing},
  doi={10.1088/2058-9565/ac22f6}
}

@article{huang2022entanglement,
  title={Entanglement swapping and quantum correlations via symmetric joint measurements},
  author={Huang, Cen-Xiao and Hu, Xiao-Min and Guo, Yu and Zhang, Chao and Liu, Bi-Heng and Huang, Yun-Feng and Li, Chuan-Feng and Guo, Guang-Can and Gisin, Nicolas and Branciard, Cyril and others},
  journal={Physical Review Letters},
  volume={129},
  number={3},
  pages={030502},
  year={2022},
  publisher={APS}
}

@article{abdi2014continuous,
  title={Continuous-variable-entanglement swapping and its local certification: Entangling distant mechanical modes},
  author={Abdi, Mehdi and Pirandola, Stefano and Tombesi, Paolo and Vitali, David},
  journal={Physical Review A},
  volume={89},
  number={2},
  pages={022331},
  year={2014},
  publisher={APS}
}

@article{pant2017rate,
  title={Rate-distance tradeoff and resource costs for all-optical quantum repeaters},
  author={Pant, Mihir and Krovi, Hari and Englund, Dirk and Guha, Saikat},
  journal={Physical Review A},
  volume={95},
  number={1},
  pages={012304},
  year={2017},
  publisher={APS}
}

@article{munro2012quantum,
  title={Quantum communication without the necessity of quantum memories},
  author={Munro, William J and Stephens, Ashley M and Devitt, Simon J and Harrison, Keith A and Nemoto, Kae},
  journal={Nature Photonics},
  volume={6},
  number={11},
  pages={777--781},
  year={2012},
  publisher={Nature Publishing Group UK London}
}

@article{sangouard2011quantum,
  title={Quantum repeaters based on atomic ensembles and linear optics},
  author={Sangouard, Nicolas and Simon, Christoph and De Riedmatten, Hugues and Gisin, Nicolas},
  journal={Reviews of Modern Physics},
  volume={83},
  number={1},
  pages={33},
  year={2011},
  publisher={APS}
}

@article{briegel1998quantum,
  title={Quantum repeaters: the role of imperfect local operations in quantum communication},
  author={Briegel, H-J and D{\"u}r, Wolfgang and Cirac, Juan I and Zoller, Peter},
  journal={Physical Review Letters},
  volume={81},
  number={26},
  pages={5932},
  year={1998},
  publisher={APS}
}

@article{gisin2007quantum,
  title={Quantum communication},
  author={Gisin, Nicolas and Thew, Rob},
  journal={Nature photonics},
  volume={1},
  number={3},
  pages={165--171},
  year={2007},
  publisher={Nature Publishing Group UK London}
}

@article{cirac1999distributed,
  title={Distributed quantum computation over noisy channels},
  author={Cirac, J Ignacio and Ekert, AK and Huelga, Susana F and Macchiavello, Chiara},
  journal={Physical Review A},
  volume={59},
  number={6},
  pages={4249},
  year={1999},
  publisher={APS}
}

@article{van2016path,
  title={The path to scalable distributed quantum computing},
  author={Van Meter, Rodney and Devitt, Simon J},
  journal={Computer},
  volume={49},
  number={9},
  pages={31--42},
  year={2016},
  publisher={IEEE}
}

@article{cuomo2020towards,
  title={Towards a distributed quantum computing ecosystem},
  author={Cuomo, Daniele and Caleffi, Marcello and Cacciapuoti, Angela Sara},
  journal={IET Quantum Communication},
  volume={1},
  number={1},
  pages={3--8},
  year={2020},
  publisher={Wiley Online Library}
}

@article{riebe2008deterministic,
  title={Deterministic entanglement swapping with an ion-trap quantum computer},
  author={Riebe, Mark and Monz, T and Kim, Kihwan and Villar, AS and Schindler, Philipp and Chwalla, M and Hennrich, Markus and Blatt, R},
  journal={Nature Physics},
  volume={4},
  number={11},
  pages={839--842},
  year={2008},
  publisher={Nature Publishing Group UK London}
}

@article{pirandola2015advances,
  title={Advances in quantum teleportation},
  author={Pirandola, Stefano and Eisert, Jens and Weedbrook, Christian and Furusawa, Akira and Braunstein, Samuel L},
  journal={Nature photonics},
  volume={9},
  number={10},
  pages={641--652},
  year={2015},
  publisher={Nature Publishing Group UK London}
}

@article{zurek2003decoherence,
  title={Decoherence, einselection, and the quantum origins of the classical},
  author={Zurek, Wojciech H},
  journal={Reviews of Modern Physics},
  volume={75},
  number={3},
  pages={715--775},
  year={2003},
  publisher={APS}
}

@article{schlosshauer2019quantum,
  title={Quantum decoherence},
  author={Schlosshauer, Maximilian},
  journal={Physics Reports},
  volume={831},
  pages={1--57},
  year={2019},
  publisher={Elsevier}
}

@article{rozpkedek2018optimizing,
  title={Optimizing practical entanglement distillation},
  author={Rozpedek, Filip and Schiet, Thomas and Elkouss, David and Doherty, Andrew C and Wehner, Stephanie and others},
  journal={Physical Review A},
  volume={97},
  number={6},
  pages={062333},
  year={2018},
  publisher={APS}
}

@article{Alittlebitofquantuminformation,
  title={A Little Bit of Quantum Information},
  author={mark Saffman},
  journal={University of Wisconsin Madison},
  year={2022},
  publisher={University of Wisconsin Madison}
}

@article{kalb2017entanglement,
  title={Entanglement distillation between solid-state quantum network nodes},
  author={Kalb, Norbert and Reiserer, Andreas A and Humphreys, Peter C and Bakermans, Jacob JW and Kamerling, Sten J and Nickerson, Naomi H and Benjamin, Simon C and Twitchen, Daniel J and Markham, Matthew and Hanson, Ronald},
  journal={Science},
  volume={356},
  number={6341},
  pages={928--932},
  year={2017},
  publisher={American Association for the Advancement of Science}
}

@article{van2008quantum,
  title={Quantum repeaters using coherent-state communication},
  author={van Loock, Peter and Lutkenhaus, Norbert and Munro, WJ and Nemoto, Kae},
  journal={Physical Review A},
  volume={78},
  number={6},
  pages={062319},
  year={2008},
  publisher={APS}
}

@article{bharti2022noisy,
  title={Noisy intermediate-scale quantum algorithms},
  author={Bharti, Kishor and Cervera-Lierta, Alba and Kyaw, Thi Ha and Haug, Tobias and Alperin-Lea, Sumner and Anand, Abhinav and Degroote, Matthias and Heimonen, Hermanni and Kottmann, Jakob S and Menke, Tim and others},
  journal={Reviews of Modern Physics},
  volume={94},
  number={1},
  pages={015004},
  year={2022},
  publisher={APS}
}

@article{stilck2021limitations,
  title={Limitations of optimization algorithms on noisy quantum devices},
  author={Stilck Fran{\c{c}}a, Daniel and Garcia-Patron, Raul},
  journal={Nature Physics},
  volume={17},
  number={11},
  pages={1221--1227},
  year={2021},
  publisher={Nature Publishing Group UK London}
}

@article{braunstein2005quantum,
  title={Quantum information with continuous variables},
  author={Braunstein, Samuel L and Van Loock, Peter},
  journal={Reviews of modern physics},
  volume={77},
  number={2},
  pages={513},
  year={2005},
  publisher={APS}
}

@article{spiller2007entanglement,
  title={Entanglement distribution for a practical quantum-dot-based quantum processor architecture},
  author={Spiller, Timothy P and D'Amico, Irene and Lovett, Brendon W},
  journal={New Journal of Physics},
  volume={9},
  number={1},
  pages={20},
  year={2007},
  publisher={IOP Publishing}
}

@article{epping2016robust,
  title={Robust entanglement distribution via quantum network coding},
  author={Epping, Michael and Kampermann, Hermann and Bruss, Dagmar},
  journal={New Journal of Physics},
  volume={18},
  number={10},
  pages={103052},
  year={2016},
  publisher={IOP Publishing}
}

@article{azuma2022quantum,
  title={Quantum repeaters: From quantum networks to the quantum internet},
  author={Azuma, Koji and Economou, Sophia E. and Elkouss, David and Hilaire, Paul and Jiang, Liang and Lo, Hoi-Kwong and Tzitrin, Ilan},
  journal={Quantum Science and Technology},
  year={2022},
  publisher={IOP Publishing},
  doi={10.1088/2058-9565/ac50a0}
}


@article{fortnow1999complexity,
  title={Complexity limitations on quantum computation},
  author={Fortnow, Lance and Rogers, John},
  journal={Journal of Computer and System Sciences},
  volume={59},
  number={2},
  pages={240--252},
  year={1999},
  publisher={Elsevier}
}

@article{wehner2018quantum,
  title={Quantum internet: A vision for the road ahead},
  author={Wehner, Stephanie and Elkouss, David and Hanson, Ronald},
  journal={Science},
  volume={362},
  number={6412},
  pages={eaam9288},
  year={2018},
  publisher={American Association for the Advancement of Science}
}

@article{caleffi2022distributed,
  title={Distributed Quantum Computing: a Survey},
  author={Caleffi, Marcello and Amoretti, Michele and Ferrari, Davide and Cuomo, Daniele and Illiano, Jessica and Manzalini, Antonio and Cacciapuoti, Angela Sara},
  journal={arXiv preprint arXiv:2212.10609},
  year={2022}
}

@article{Wang2022QuantumMemory,
  title={Field-deployable Quantum Memory for Quantum Networking},
  author={Wang, Yang and Craddock, Alexander N. and Sekelsky, Rourke and Flament, Mael and Namazi, Mehdi},
  year={2022},
  address={Brooklyn, NY},
  note={Qunnect Inc., 141 Flushing Ave, Ste 1110, Brooklyn, NY 11205-1005},
  date={September 9}
}

@article{Bogdanov2019QuantumPlasmonics,
  title={Overcoming quantum decoherence with plasmonics: The use of nanoscale plasmonic metamaterials to optimize photon-matter interactions},
  author={Bogdanov, Simeon I. and Boltasseva, Alexandra and Shalaev, Vladimir M.},
  journal={Science},
  volume={364},
  issue={6440},
  year={2019},
  publisher={AAAS},
  doi={10.1126/science.aax3766},
  url={https://www.science.org/doi/10.1126/science.aax3766},
  note={Published by AAAS, sciencemag.org}
}
@article{Drmota2023QuantumMemory,
  title={Robust Quantum Memory in a Trapped-Ion Quantum Network Node},
  author={Drmota, P. and Main, D. and Nadlinger, D. P. and Nichol, B. C. and Weber, M. A. and Ainley, E. M. and Agrawal, A. and Srinivas, R. and Araneda, G. and Ballance, C. J. and Lucas, D. M.},
  journal={Physical Review Letters},
  volume={130},
  pages={090803},
  year={2023},
  publisher={American Physical Society},
  doi={10.1103/PhysRevLett.130.090803},
  url={https://link.aps.org/doi/10.1103/PhysRevLett.130.090803},
  note={Published 3 March 2023}
}
@article{Wille2019Majorana,
  title={Simulating topological tensor networks with Majorana qubits},
  author={Wille, C. and Egger, R. and Eisert, J. and Altland, A.},
  journal={Physical Review B},
  volume={99},
  pages={115117},
  year={2019},
  publisher={American Physical Society},
  doi={10.1103/PhysRevB.99.115117},
  url={https://link.aps.org/doi/10.1103/PhysRevB.99.115117},
  note={Published 14 March 2019}
}

@article{Lashgari2013TimelyThroughput,
  title={Timely Throughput of Heterogeneous Wireless Networks: Fundamental Limits and Algorithms},
  author={Sina Lashgari and A. Salman Avestimehr},
  journal={IEEE Transactions on Information Theory},
  volume={59},
  number={12},
  pages={8414--8433},
  year={2013},
  month={Dec},
  publisher={IEEE},
  doi={10.1109/TIT.2013.2283492},
  ISSN={},
  abstract={The proliferation of different wireless access technologies, together with the growing number of multi-radio wireless devices suggest that the opportunistic utilization of multiple connections at the users can be an effective solution to the phenomenal growth of traffic demand in wireless networks. In this paper, we consider the downlink of a wireless network with N access points (APs) and M clients, where each client is connected to several out-of-band APs, and requests delay-sensitive traffic (e.g., real-time video). We adopt the framework of Hou and study the maximum total timely throughput of the network, denoted by CT3, which is the maximum average number of packets delivered successfully before their deadline. ...},
  note={Published online: 25 September 2013}
}

@inproceedings{Llopis2016MinimizingLatency,
  title={Minimizing Latency of Critical Traffic through SDN},
  author={Joan Meseguer Llopis and Janusz Pieczerak and Tomasz Janaszka},
  booktitle={2016 IEEE International Conference on Networking, Architecture and Storage (NAS)},
  pages={},
  year={2016},
  month={Aug},
  publisher={IEEE},
  doi={10.1109/NAS.2016.7549408},
  address={Long Beach, CA, USA},
  isbn={},
  note={Conference date: 08-10 August 2016; published online: 25 August 2016}
}
@article{GhaniAlJobouri2023PacketLoss,
  title={Packet Loss Optimization in Router Forwarding Tasks Based on the Particle Swarm Algorithm},
  author={Rana Fareed Ghani and Laith Al-Jobouri},
  journal={Electronics},
  volume={12},
  number={2},
  pages={462},
  year={2023},
  doi={10.3390/electronics12020462},
  publisher={MDPI},
  address={Baghdad 10066, Iraq; Dundee DD1 1HG, UK},
  note={Submission received: 5 November 2022 / Revised: 6 January 2023 / Accepted: 11 January 2023 / Published: 16 January 2023},
  url={https://doi.org/10.3390/electronics12020462}
}
@article{LanjewarGuptaAODV,
  title={Optimizing Cost, Delay, Packet Loss and Network Load in AODV Routing Protocol},
  author={Ashutosh Lanjewar and Neelesh Gupta},
  journal={},
  year={},
  note={(1) M.Tech. Student, Digital Communication, T.I.E.I.T (TRUBA), BHOPAL (M.P.)-India, (2) Electronics and Communication, T.I.E.I.T (TRUBA), BHOPAL (M.P.)-India},
  abstract={AODV is Ad-hoc On-Demand Distance Vector. A mobile ad-hoc network (MANET) is a self-configuring network of mobile devices connected by wireless, without any fixed infrastructure. The dynamic nature of MANETs presents challenges in maintaining optimal performance metrics such as packet loss, end-to-end delay, and network load. This paper focuses on improving these metrics within the AODV routing protocol, using NS-2 for simulation purposes.}
}
@article{BreslauEstrinFallFloydHeidemannHelmyHuangMcCanneVaradhanXuYu2023Advances,
  title={Advances in Network Simulation},
  author={L. Breslau and D. Estrin and K. Fall and S. Floyd and J. Heidemann and A. Helmy and P. Huang and S. McCanne and K. Varadhan and Ya Xu and Haobo Yu},
  journal={IEEE},
  year={2000},
  note={},
  abstract={},
  url={}
}

@article{mit_harvard_2020,
  author = {Hamilton, D. and Dixon, B.},
  title = {Quantum repeaters use defects in diamond to interconnect quantum systems},
  journal = {MIT News},
  year = {2020},
  url = {https://news.mit.edu/2020/quantum-repeaters-diamond-defects-1217}
}

@article{innsbruck_2023,
  author = {Krutyanskiy, V. and Pompili, M. and van Leent, T. and Langenfeld, S. and Beukers, H. and Humphreys, P. C. and Hanson, R.},
  title = {Telecom-wavelength quantum repeater node based on a trapped-ion processor},
  journal = {Physical Review Letters},
  year = {2023},
  volume = {130},
  number = {213601},
  url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.130.213601}
}
@article{PhysRevA.71.060310,
  title = {Efficient high-fidelity quantum computation using matter qubits and linear optics},
  author = {Barrett, Sean D. and Kok, Pieter},
  journal = {Phys. Rev. A},
  volume = {71},
  issue = {6},
  pages = {060310},
  numpages = {4},
  year = {2005},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.71.060310},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.71.060310}
}

@misc{aliro_quantum_memories_2024,
  title        = {Quantum Memories for Quantum Networking},
  author       = {Aliro Quantum},
  year         = {2024},
  url          = {https://www.aliroquantum.com/quantum-memories-for-quantum-networking},
}

@article{Ruf2021Quantum,
  title={Quantum networks based on color centers in diamond},
  author={Ruf, Maximilian and Wan, Noel H. and Choi, Hyeongrak and Englund, Dirk and Hanson, Ronald},
  journal={Journal of Applied Physics},
  volume={130},
  number={7},
  pages={070901},
  year={2021},
  publisher={AIP Publishing},
  doi={10.1063/5.0056534},
  url={https://doi.org/10.1063/5.0056534}
}
@article{Aguado2020Majorana,
  title={Majorana qubits for topological quantum computing},
  author={Aguado, Ramón and Kouwenhoven, Leo P.},
  journal={Physics Today},
  volume={73},
  number={6},
  pages={44--50},
  year={2020},
  publisher={AIP Publishing},
  doi={10.1063/PT.3.4499},
  url={https://doi.org/10.1063/PT.3.4499}
}
@article{Dey2020Quantum,
  title={Quantum Game Theory Meets Quantum Networks},
  author={Dey, Indrakshi and Marchetti, Nicola and Caleffi, Marcello and Cacciapuoti, Angela Sara},
  journal={IEEE},
  year={2020},
  publisher={IEEE}
}
@article{Wang2022Entangled,
  title={Arbitrary entangled state transfer via a topological qubit chain},
  author={Wang, Chong and Li, Linhu and Gong, Jiangbin and Liu, Yu-xi},
  journal={Physical Review A},
  volume={106},
  number={052411},
  pages={052411},
  year={2022},
  publisher={American Physical Society},
  doi={10.1103/PhysRevA.106.052411},
  url={https://link.aps.org/doi/10.1103/PhysRevA.106.052411}
}
@INPROCEEDINGS{9796816,
  author={Farahbakhsh, Ali and Feng, Chen},
  booktitle={IEEE INFOCOM 2022 - IEEE Conference on Computer Communications}, 
  title={Opportunistic Routing in Quantum Networks}, 
  year={2022},
  volume={},
  number={},
  pages={490-499},
  keywords={Quantum entanglement;Conferences;Routing;Quantum networks},
  doi={10.1109/INFOCOM48880.2022.9796816}}
@inproceedings{Chehimi2021Entanglement,
  title={Entanglement rate optimization in heterogeneous quantum communication networks},
  author={Chehimi, M. and Saad, W.},
  booktitle={2021 17th International Symposium on Wireless Communication Systems (ISWCS)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}
@article{Rozpedek2019NearTerm,
  title={Near-term quantum-repeater experiments with nitrogen-vacancy centers: Overcoming the limitations of direct transmission},
  author={Rozpedek, F. and others},
  journal={Physical Review A},
  volume={99},
  number={5},
  pages={052330},
  year={2019},
  publisher={American Physical Society},
  doi={10.1103/PhysRevA.99.052330}
}
@article{PhysRevResearch.3.013279,
  title = {Limits and security of free-space quantum communications},
  author = {Pirandola, Stefano},
  journal = {Phys. Rev. Res.},
  volume = {3},
  issue = {1},
  pages = {013279},
  numpages = {33},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.3.013279},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.3.013279}
}
@article{PhysRevLett.128.150502,
  title = {Optimal Entanglement Swapping in Quantum Repeaters},
  author = {Shchukin, Evgeny and van Loock, Peter},
  journal = {Phys. Rev. Lett.},
  volume = {128},
  issue = {15},
  pages = {150502},
  numpages = {5},
  year = {2022},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.128.150502},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.128.150502}
}
@article{Chen2023Scalable,
  title={Scalable and programmable phononic network with trapped ions},
  author={Chen, W. and Lu, Y. and Zhang, S. and others},
  journal={Nature Physics},
  volume={19},
  pages={877--883},
  year={2023},
  doi={10.1038/s41567-023-01952-5},
  url={https://doi.org/10.1038/s41567-023-01952-5}
}





